Reinforcement Learning-Based Model Matching in COBRA, a Slithering Snake Robot

This work employs a reinforcement learning-based model identification method aimed at enhancing the accuracy of the dynamics for our snake robot, called COBRA. Leveraging gradient information and iterative optimization, the proposed approach refines the parameters of COBRA's dynamical model such as coefficient of friction and actuator parameters using experimental and simulated data. Experimental validation on the hardware platform demonstrates the efficacy of the proposed approach, highlighting its potential to address sim-to-real gap in robot implementation.

==> Makefile <==
# ------------------------------------------------------------------------
# Makefile:
# ------------------------------------------------------------------------
# written by:	Gunar Schirner 
# External References:
#   http://kriemhild.uft.uni-bremen.de/viewvc/vim/Makefile.pdflatex
#   http://www.tex.ac.uk/tex-archive/help/uk-tex-faq/Makefile
# last update:	$id$
#
# Help screen (start every help line with #h)
#
#h make        builds ALL_REF
#h
#h make publish 
#h             publish the build output to HTML publish directory  
#h
# --- names --------------------------------------------------------------

PROJECT	=	thesis

SRCNAME	=	$(PROJECT)_SRC.tar.gz
BINNAME	=	$(PROJECT)_BIN.tar.gz
ORIG	=	

TMP	=	/tmp
# own name
MAKEF   =       Makefile

# path for automatic publishing, put into your public_html directory`
PUBLISH_PATH = /home/student/<studentName>/public_html/thesis
VERSION_FILE = svnRev.tex

# set automatically by hook script (Post commit hook)
# SVN_REPO_PATH 
# SVN_REV

# --- lists --------------------------------------------------------------

ALL	=	$(PROJECT).pdf



# auto use all *.tex file in the own and in pi directory as dependency input 
INCLUDE	:=	$(shell [ -d tex ] && echo tex/*.tex )

SOURCES =	$(PROJECT).tex	\
		$(INCLUDE)

#BIBFILES :=  macro/bib-strings.bib macro/IEEEabrv.bib $(shell [ -d bib ] && echo bib/*.bib )

FIGFILES =

PPTFILES =	

PRNFILES =

# auto use all *.eps files in the fig directory as a dependency input 
#  FIGURES directory may not exist
# uncomment once first eps is added 
EPSFILES :=	$(shell [ -d fig ] && echo fig/*.eps) 


# auto use all *.pdf files in the fig directory as a dependency input 
#  FIGURES directory may not exist
# uncomment once first pdf is added 
#PDFFIGS :=	$(shell [ -d fig ] && echo fig/*.pdf) 


FIGURES	=	$(EPSFILES:.eps=.pdf) $(PDFFIGS)

#MACROS	=	macro/macros.tex

OTHERS	=	Makefile	


ORIGS	=	$(SOURCES) $(MACROS) $(OTHERS)

SRCTAR	=	$(SOURCES) $(MACROS) $(OTHERS)	\
		$(FIGFILES) $(PPTFILES) $(PRNFILES) $(EPSFILES)

BINTAR	=	$(ALL)

# --- environment --------------------------------------------------------

TEXINPUTS =	TEXINPUTS=.:MACROS:

TEXENV	=	$(TEXINPUTS)

# --- commands -----------------------------------------------------------

FIGPS	=	fig2dev -L ps
PRN2EPS	=	PATH=bin:$$PATH prn2eps
LATEX	=	$(TEXENV) latex
PDFLATEX =      pdflatex --interaction nonstopmode
BIBTEX	=	bibtex
DVIPS	=	dvips -Z -D 600 -t letter -Ppdf
PS2PDF	=	ps2pdf
EPS2PDF	=	epstopdf
PSSEL	=	psselect
TAR	=	gtar cvzf
RM	=	rm -f
MV	=	mv -f
MAKEIDX	=	makeindex
GV	=	ghostview
ECHO	=	echo
GREP	=	grep
WC	=	wc
CD	=	cd
CAT	=	cat
XLESS	=	xless
SPELL	=	nspell -t
SORT	=	sort -f
MAKEIDX	=	makeindex
DISTILL =       GS_OPTIONS="-dAutoFilterColorImages=false \
                            -dColorImageFilter=/FlateEncode" ps2pdf14
THUMBPDF=       thumbpdf --modes=dvips

# parse string to cause rebuild of latex
RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right|Table widths have changed. Rerun LaTeX.|Linenumber reference failed)"

# parse string to cause rebuild of bibtex
RERUNBIB = "No file.*\.bbl|Citation.*undefined"



# --- general rules ------------------------------------------------------

.SUFFIXES:
.SUFFIXES:	.fig .ps .prn .eps .tex .bbl .pdf

.fig.ps:
	$(FIGPS) $*.fig $*.ps

.prn.eps:
	$(PRN2EPS) $*.prn $*.eps

#GS added automatic conversion for eps files, epstopdf packages seems
# not installed on this linux installation
.eps.pdf:
	$(EPS2PDF) $*.eps

.tex.bbl:
	$(LATEX) $*.tex
	$(BIBTEX) $*

# run pdflatex once and bib + subsequent pdflatex conditionally
%.pdf: %.tex
	$(PDFLATEX) $<
	@egrep -c $(RERUNBIB) $*.log && (bibtex $*;$(PDFLATEX) $<); true
	@egrep $(RERUN) $*.log && ($(PDFLATEX) $<) ; true
	@egrep $(RERUN) $*.log && ($(PDFLATEX) $<) ; true


# --- rules --------------------------------------------------------------

all:		$(ALL)

# automatically produce help message by grep for sepcial comment lines 
help:;	@sed -n -e 's/^#h//p'  < $(MAKEF) | sed -e 's/ALL_REF/$(ALL)/g'

# second phase of the publish requires to get the current SVN version 
ifdef SECOND_PHASE
SVN_REV := $(shell svn info | sed -n -e 's/.*Revision: //p')
endif

# debug rule to print current version 
echo_ver:
	@echo $(SVN_REV)

# paste the current version information into tex file so that it 
# can be included into build
create_version_file: 
	@echo "\\newcommand{\\svnRevRef}{$(SVN_REV)}" > $(VERSION_FILE)


# actual publishing action 
autobuild_publish_2nd: create_version_file
	make >  $(PUBLISH_PATH)/z_buildlog.r$(SVN_REV).log
	set -e ; for f in $(basename $(filter %.pdf, $(ALL))); do        \
		rm -f $(PUBLISH_PATH)/$$f.r*.pdf;                         \
		cp $$f.pdf $(PUBLISH_PATH)/$$f.r$(SVN_REV).pdf;   \
		rm -f $(PUBLISH_PATH)/$$f.pdf; \
		ln -s $(PUBLISH_PATH)/$$f.r$(SVN_REV).pdf $(PUBLISH_PATH)/$$f.pdf ;  \
	done

# if the revision is already passed in as a parameter, we do not 
# need to trieve it again 
ifneq ("$(SVN_REV)", "")
# clean update build and publish 
publish: clean svn_up autobuild_publish_2nd
else
# cleanup, svn update and kick off second phase
publish: 
	make clean
	svn up
	make autobuild_publish_2nd SECOND_PHASE=1
endif

# helper rule to call svn update 
svn_up: 
	svn up


clean:
	$(RM) $(ALL)
	$(RM) *.ps *.pdf
	$(RM) *.dvi
	$(RM) *.toc *.lot *.lof *.log *.aux
	$(RM) *.idx *.ind *.ilg
	$(RM) *.inx *.srt
	$(RM) *.blg *.bbl
	$(RM) *.out
	$(RM) *.BAK *.bak *~
	$(RM) macro/*.BAK macro/*.bak macro/*~
	$(RM) texput.log
	$(RM) $(ORIG)

tar:
	-$(MV) $(SRCNAME) $(SRCNAME).bak
	-$(MV) $(BINNAME) $(BINNAME).bak
	-$(TAR) $(SRCNAME) $(SRCTAR)
	-$(TAR) $(BINNAME) $(BINTAR)

spell:
	$(SPELL) $(SOURCES)

orig:	$(ORIG)

todo:	$(ORIG)
	-$(GREP) -n "\.\.\.\." `$(CAT) $(ORIG)` >$(TMP)/todo
	$(WC) -l $(TMP)/todo ; $(XLESS) $(TMP)/todo ; $(RM) $(TMP)/todo &

1:
	$(LATEX) $(PROJECT).tex
	$(DVIPS) $(PROJECT).dvi -o $(PROJECT).ps

2:
	$(LATEX) $(PROJECT).tex
	$(LATEX) $(PROJECT).tex
	$(DVIPS) $(PROJECT).dvi -o $(PROJECT).ps


# --- project rules ---

$(PROJECT).pdf:  $(PROJECT).tex $(MACROS) $(INCLUDE) $(FIGURES) $(BIBFILES) 


summary.pdf:	summary.tex

$(PROJECT).ps: $(PROJECT).pdf
	pdf2ps $<

Description.ps: $(PROJECT).ps
	$(PSSEL) 1-15 $(PROJECT).ps Description.ps

Description.pdf:	Description.ps
	$(DISTILL) Description.ps Description.pdf


References.ps: $(PROJECT).ps
	$(PSSEL) 16- $(PROJECT).ps References.ps

References.pdf:	References.ps
	$(DISTILL) References.ps References.pdf


# --- other rules ---

$(ORIG):	$(ORIGS)
	$(ECHO) >$(ORIG) $(ORIGS)



#h dbgPrint   VAR=<varName> print content of variable <varName>
dbgPrint:
	@echo "$(VAR)=$($(VAR))"
# --- EOF ----------------------------------------------------------------


==> tex/cobrasim2real.tex <==
\chapter{Simulation-to-Reality Gap in COBRA}
\label{chap:sim2real_cobra}

\section{COBRA Platform}
\begin{figure}
  \centering
  \includegraphics[width=1.0\linewidth]{fig/fbd.png} 
  \caption{Illustrates free body diagram of the \ac{COBRA} platform}
  \label{fig:fbd}
\end{figure}

COBRA, an acronym for Crater Observing Bio-inspired Rolling Articulator, is a snake robot designed after the intricate locomotion of serpentine creatures \cite{salagame_how_2023} \cite{rollinson_gait-based_2013} \cite{mori_reinforcement_nodate}. This robot is specifically engineered to navigate and endure rugged terrains and environments, such as craters, where traditional wheeled or legged robots may struggle. Figure \ref{fig:fbd} shows a free body diagram of the COBRA platform and the ground coefficients of friction. With 11 joints and 12 links, the COBRA platform exhibits a complex mechanical structure that allows for versatile movements and functionalities. The presence of 6 yawing joints and 5 pitching joints enables the platform to achieve a wide range of orientations and configurations, making it suitable for diverse applications in robotics and engineering.

The free body diagram provides a detailed representation of the forces and moments acting on the COBRA platform as it interacts with the ground. The coefficients of friction play a crucial role in analyzing the stability and motion dynamics of the platform during various maneuvers.

\begin{equation}
    \begin{aligned}
        \left[\begin{array}{cc}
D_H & D_{H a} \\
D_{a H} & D_a
\end{array}\right]\left[\begin{array}{l}
\ddot{q}_H \\
\ddot{q}_a
\end{array}\right]&+\left[\begin{array}{l}
H_H \\
H_a
\end{array}\right]=\left[\begin{array}{l}
0 \\
B_a
\end{array}\right]u+\\&
+
\left[\begin{array}{cc}
J_{H}^\top \\ J_{a}^\top
\end{array}\right]F_{GRF}
    \end{aligned}
\label{eq:full-dynamics}
\end{equation}
\noindent where $D_i$, $H_i$, $B_i$, and $J_i$ are partitioned model parameters corresponding to the head 'H' and actuated 'a' joints. $F_{GRF}$ denotes the ground reaction forces. $u$ embodies the joint actuation torques. The actuator parameters include: transmission inertia, internal damping, and dc motor constant. The reference trajectories used in the actuator models are generated by 
% \begin{equation}
% \begin{aligned}
%     y(t) = A \sin(\omega t + \phi)
% \end{aligned}
% \label{eq:cpg}
% \end{equation}
% \noindent where \( y(t) \) represents the lateral position of the COBRA platform at time \( t \), \( A \) is the amplitude of the sidewinding motion, \( \omega \) is the angular frequency, and \( \phi \) is the phase angle.

The sidewinding motion depicted in Fig. \ref{fig:disparity} demonstrates the platform's capability to traverse terrain with varying obstacles and inclines. By utilizing a sine-based trajectory, the COBRA platform can adapt its movement to navigate through complex environments while maintaining stability and efficiency. The parameters \( A \), \( \omega \), and \( \phi \) in the sine equation allow for precise control over the sidewinding motion, enabling the platform to adjust its speed, direction, and curvature as needed. This flexibility is crucial for applications such as search and rescue missions, exploration of uneven terrains, and inspection tasks in challenging environments.

The ground model used in our simulations is given by 
%
\begin{equation}
\begin{aligned}
    F_{GRF} &= \begin{cases} \, 0 ~~  \mbox{if } p_{C,z} > 0  \\
     [F_{GRF,x},\, F_{GRF,y},\, F_{GRF,z}]^\top ~~ \mbox{else} \end{cases} \\
\end{aligned}
\label{eq:grf}
\end{equation}
\noindent where $p_{C,i},~~i=x,y,z$ are the $x-y-z$ positions of the contact point; $F_{GRF,i},~~i=x,y,z$ are the $x-y-z$ components of the ground reaction force assuming a contact takes place between the robot and the ground substrate. In Eq.~\ref{eq:grf}, the force terms are given by 
\begin{equation}
     F_{GRF,z} = -k_1 p_{C,z} - k_{2} \dot p_{C,z}, 
    \label{eq:grf-z}
\end{equation}
% \noindent and 
\begin{equation}
    F_{GRF,i} = - s_{i} F_{GRF,z} \, \mathrm{sgn}(\dot p_{C,i}) - \mu_v \dot p_{C,i} ~~  \mbox{if} ~~i=x, y
    \label{eq:grf-xy}
\end{equation}
\noindent In Eqs.~\ref{eq:grf-z} and \ref{eq:grf-xy}, $k_{1}$ and $k_{2}$ are the spring and damping coefficients of the compliant surface model. In Eq.~\ref{eq:grf-xy}, the term $s_i$ is given by 
\begin{equation}
    s_{i} = \Big(\mu_c - (\mu_c - \mu_s) \mathrm{exp} \left(-|\dot p_{C,i}|^2/v_s^2  \right) \Big)
    \label{eq:grf-s}
\end{equation}
\noindent where $\mu_c$, $\mu_s$, and $\mu_v$ are the Coulomb, static, and viscous friction coefficients; and, $v_s > 0$ is the Stribeck velocity. Specifically speaking, from Eqs.~\ref{eq:full-dynamics} and \ref{eq:grf}, the following parameters are unknown to us: actuator models parameters and Stribeck terms \cite{liljeback_simplified_2010}.

% \begin{figure}
%   \centering
%   \includegraphics[width=1.0\linewidth]{fig/latest_sidewinding.png} 
%   \caption{}
%   \label{fig:sidewind}
% \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[width=0.9\linewidth]{fig/3d_traj_robot.png} 
%   \caption{}
%   \label{fig:3dtraj}
% \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[width=0.9\linewidth]{fig/joint_traj_robot.png} 
%   \caption{}
%   \label{fig:jointtraj}
% \end{figure}

% \section{Sidewinding Experiment}

% Figure \ref{fig:sidewind} shows the COBRA platform sidewinding on a flat ground. The sidewinding trajectory is generated by the sine equation \ref{eq:cpg}. \ref{fig:disparity} hightlights the simulaton-to-reality gap observed in the Webots simulator. Experiments were conducted on the physical robot, and data were collected using motion capture technology to precisely record the trajectories of the head, tail, and middle links. Additionally, joint trajectory data for all eleven joints were recorded. The odd-numbered joints (1, 3, 5, ..., 11 from the head) executed pitching motions, while the even-numbered joints (2, 4, ..., 10 from the head) executed yawing motions. A sidewinding gait was generated by applying a sinusoidal input signal to each joint, serving as a standard input with adjustable parameters to modify the robot's behavior. The input signal followed a sine-wave pattern based on Equation 2, with varying phase differences applied to each joint.
% $$
% A_\text{pitching} = 14^\circ,~A_\text{yawing} = 60^\circ
% $$
% $$
% \phi = \frac{\pi}{2}[0, 0, 1, 1, 2, 2, 3, 3, 0, 0, 1]
% $$

% \section{Simulation-to-Reality Gap}

% The identical trajectory is also executed within the Webots simulator, allowing us to observe the discrepancy or gap, as shown in Figure \ref{fig:disparity}, between the simulator and the actual robot. This disparity is more evident in Figures \ref{fig:sim2real_head_trajectories}, where I compare the head trajectories over time for three different gait patterns in both the actual robot and the base simulator (untuned model). Gait 1 represents a sidewinding motion at 0.35 Hz, Gait 2 is sidewinding at 0.5 Hz, and Gait 3 is a sidewinding motion at 0.65 Hz. Additionally, Figure \ref{fig:sim2real_joint_angles} offers insights into how the performance of actuator model also contributes to the gap observed between simulation and reality. These disparities hinder the seamless transfer of control policies developed in simulation to the real robot, limiting the effectiveness of learned behaviors in practical applications. Hence, addressing the sim-to-real issue is crucial for ensuring the reliability and robustness of COBRA when deployed in diverse and dynamic environments.

% \begin{figure}
%   \centering
%   \includegraphics[width=0.7\linewidth]{fig/disparity.png} 
%   \caption{}
%   \label{fig:disparity}
% \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[width=1.0\linewidth]{fig/sim2real_head_trajectories.png} 
%   \caption{}
%   \label{fig:sim2real_head_trajectories}
% \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[width=1.0\linewidth]{fig/sim2real_joint_angles.png} 
%   \caption{}
%   \label{fig:sim2real_joint_angles}
% \end{figure}

\section{Model Matching}

My strategy to address the sim2real gap involves employing the Reinforcement Learning-based Model Matching approach. This method aims to identify the accurate parameters of COBRA's dynamic model within the simulation environment, thus bridging the gap between simulation and reality. By leveraging these precise parameters, we can develop and train advanced locomotion and manipulation strategies using learning-based techniques. These strategies can then be effectively transferred and implemented on the real robot, enhancing its performance and capabilities.
